A Conformal Approach to Feature-based Newsvendor under Model Misspecification

In many data-driven decision-making problems, performance guarantees often depend heavily on the correctness of model assumptions, which may frequently fail in practice. We address this issue in the context of a feature-based newsvendor problem, where demand is influenced by observed features such as demographics and seasonality. To mitigate the impact of model misspecification, we propose a model-free and distribution-free framework inspired by conformal prediction. Our approach consists of two phases: a training phase, which can utilize any type of prediction method, and a calibration phase that conformalizes the model bias. To enhance predictive performance, we explore the balance between data quality and quantity, recognizing the inherent trade-off: more selective training data improves quality but reduces quantity. Importantly, we provide statistical guarantees for the conformalized critical quantile, independent of the correctness of the underlying model. Moreover, we quantify the confidence interval of the critical quantile, with its width decreasing as data quality and quantity improve. We validate our framework using both simulated data and a real-world dataset from the Capital Bikeshare program in Washington, D.C. Across these experiments, our proposed method consistently outperforms benchmark algorithms, reducing newsvendor loss by up to 40% on the simulated data and 25% on the real-world dataset.

==> arxiv.tex <==
\SingleSpacedXI

\setlength{\parskip}{1ex}
\renewcommand{\theARTICLETOP}{}
\renewcommand{\theARTICLERULE}{\vspace{12pt}}
\renewcommand{\theRRHFirstLine}{}
\renewcommand{\theRRHSecondLine}{}
\renewcommand{\theLRHFirstLine}{}
\renewcommand{\theLRHSecondLine}{}
\renewcommand{\theECLRHFirstLine}{}%
\renewcommand{\theECLRHSecondLine}{}%
\renewcommand{\theECRRHFirstLine}{}%
\renewcommand{\theECRRHSecondLine}{}%
\renewcommand{\endproof}{\endTrivlist\addvspace{2ex}}
\makeatletter
\renewcommand\section{\@startsection {section}{1}{\z@}{-13pt plus -6pt minus -3pt}{4pt}%
  {\fs.13.15.\bfseries\RAGG}}%
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}{-13pt plus -6pt minus -3pt}{4pt}%
  {\TEN\bfseries\RAGG}}%
\makeatother

\usepackage[scaled=.98,sups,osf]{XCharter}% lining figures in math, osf in text 
% \usepackage[scaled=1.04,varqu,varl]{inconsolata}% inconsolata typewriter 
% \usepackage[type1]{cabin}% sans serif 
\usepackage[charter,vvarbb,scaled=1.05]{newtxmath} 
\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}
% \let\mathfrak\undefined
% \usepackage{eufrak}
% \DeclareMathAlphabet\mathfrak{U}{euf}{m}{n}
% \SetMathAlphabet\mathfrak{bold}{U}{euf}{b}{n}
\usepackage[scaled=0.95]{helvet}
% \SetSymbolFont{letters}{normal}{OML}{mdbch}{m}{it}
% \SetMathAlphabet{\mathsf}{bold}{OT1}{lmss}{bx}{n}

